Adaptive Neural Network-based Unscented Kalman Filter for Robust Pose Tracking of Noncooperative Spacecraft

This paper presents a neural network-based Unscented Kalman Filter (UKF) to estimate and track the pose (i.e., position and orientation) of a known, noncooperative, tumbling target spacecraft in a close-proximity rendezvous scenario. The UKF estimates the target's orbit and attitude relative to the servicer based on the pose information provided by a multi-task Convolutional Neural Network (CNN) from incoming monocular images of the target. In order to enable reliable tracking, the process noise covariance matrix of the UKF is tuned online using adaptive state noise compensation which leverages a newly developed closed-form process noise model for relative attitude dynamics. This paper also introduces the Satellite Hardware-In-the-loop Rendezvous Trajectories (SHIRT) dataset to enable comprehensive analyses of the performance and robustness of the proposed pipeline. SHIRT comprises the labeled images of two representative rendezvous trajectories in low Earth orbit created using both a graphics renderer and a robotic testbed. Specifically, the CNN is solely trained on synthetic data, whereas functionality and performance of the complete navigation pipeline are evaluated on real images from the robotic testbed. The proposed UKF is evaluated on SHIRT and is shown to have sub-decimeter-level position and degree-level orientation errors at steady-state.

==> sections/04_backup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Analytical Process Noise Models
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analytical Process Noise Models} \label{sec:Process Noise Modeling}

In order to perform ASNC to adaptively tune the process noise covariance matrix, the process noise model must be derived for the state vector described in Eq.~\ref{eqn:state_vector}. In this work, the noise components of the orbital and attitude states are decoupled to facilitate the derivation and computation, i.e., 
\begin{align}
	\bm{Q}_k = \begin{bmatrix} \bm{Q}_{\roe, k} & \bm{0}_{6 \times 6} \\ \bm{0}_{6 \times 6} & \bm{Q}_{\bm{q}, k} \end{bmatrix}.
\end{align}
The process noise power spectral density matrix for the unmodeled relative cartesian accelerations is modeled in the servicer's RTN frame, whereas that of the unmodeled differential angular accelerations is modeled about the target's principal axes. For simplicity, the process noise power spectral density matrices for both relative orbit and attitude states are assumed diagonal,
\begin{align}
	\bm{\widetilde{Q}}_{\roe}= \begin{bmatrix} \widetilde{Q}_{\roe}^r & 0 & 0 \\ 0 & \widetilde{Q}_{\roe}^t & 0 \\ 0 & 0 & \widetilde{Q}_{\roe}^n \end{bmatrix}, ~~ \bm{\widetilde{Q}}_{\bm{q}} = \begin{bmatrix} \widetilde{Q}_{\bm{q}}^x & 0 & 0 \\ 0 & \widetilde{Q}_{\bm{q}}^y & 0 \\ 0 & 0 & \widetilde{Q}_{\bm{q}}^z \end{bmatrix}.
\end{align}
Then, taking the ROE state as an example, the process noise covariance matrix in Eq.~\ref{eqn:Q_eq} becomes
\begin{align} \label{eqn:Q_roe as sum of diagonal}
	\bm{Q}_{\roe, k} = \bm{X}_{k}^r\widetilde{Q}_{\roe,k}^r + \bm{X}_{k}^t\widetilde{Q}_{\roe,k}^t + \bm{X}_{k}^n\widetilde{Q}_{\roe,k}^n,
\end{align}
where 
\begin{align} \label{eqn:X matrix def - general}
	\bm{X}_{k}^i = \int_{t_{k-1}}^{t_k} \bm{\bar{\Gamma}}_{k}^i(t_k ,\tau) \bm{\bar{\Gamma}}_{k}^i(t_k ,\tau)^\top d\tau, ~~~ i \in \{r, t, n\}.
\end{align}
Here, $\bm{\bar{\Gamma}}_k(t_k, t) = [\bm{\bar{\Gamma}}_{k}^r$~~~$\bm{\bar{\Gamma}}_{k}^t$~~~$\bm{\bar{\Gamma}}_{k}^n] = \bm{\Phi}(t_k, t) \bm{\Gamma}_k(t)$. Equations \ref{eqn:Q_roe as sum of diagonal} and \ref{eqn:X matrix def - general} can now be used to construct the linear mapping of Eq.~\ref{eqn:ASNC linear mapping} as
\begin{align} \label{eqn:ASNC Linear Mapping Expanded}
	\bm{Q}_{\delta\bm{\alpha}, k}^\text{vech} = \bm{X}_k \bm{\widetilde{Q}}_{\roe,k}^\text{diag} = \begin{bmatrix} \vert & \vert & \vert \\ \text{vech}(\bm{X}_{k}^r) & \text{vech}(\bm{X}_{k}^t) & \text{vech}(\bm{X}_{k}^n) \\ \vert & \vert & \vert \end{bmatrix} \begin{bmatrix} \widetilde{Q}_{\roe,k}^r \\ \widetilde{Q}_{\roe,k}^t \\ \widetilde{Q}_{\roe,k}^n \end{bmatrix}.
\end{align}
A similar expression can be constructed for the attitude dynamics as well. Once $\bm{X}_k$ matrices can be constructed from Eq.~\ref{eqn:ASNC Linear Mapping Expanded} for both ROE and attitude states, the weighted least-squares minimization problem of Eq.~\ref{eqn:ASNC LS minimizaiton} can be solved individually for both states using an off-the-shelf least-squares or quadratic programming solver. In this work, MATLAB's \texttt{lsqlin} command is used to solve Eq.~\ref{eqn:ASNC LS minimizaiton} with a non-negativity constraint, i.e., $\bm{\widetilde{Q}}_\ell^\text{diag} = \bm{0}_{3 \times 1}$ to ensure a positive semi-definite solution.

The sections below describe the analytical process noise covariance models for both states. The derivation of the model for the attitude motion is a new and essential contribution of this work.

%%%%%%%%%%%%%%%%%%%%%%
\subsection{ROE State Process Noise}

For a nonsingular ROE representation based on the equinoctial elements, \citet{Stacey2022CovModel} derived the process noise covariance model under the assumption of two-body motions. Specifically, for a small separation between two spacecraft, the authors first derive the process noise $\bm{Q}_{\roe^\prime}$ for an alternative ROE representation defined as $\roe^\prime = \bm{\alpha}_T - \bm{\alpha_S}$. Then, the process noise for nonsingular ROE can be recovered via
\begin{align} \label{eqn:Q from OE diff to NS ROE}
	\bm{Q}_{\delta\bm{\alpha}, k} = \bm{J}_{\delta\bm{\alpha}}(t_k) \bm{Q}_{\delta\bm{\alpha}^\prime, k} \bm{J}_{\delta\bm{\alpha}}(t_k)^\top,
\end{align}
where 
\begin{align} \label{eqn:J from OE diff to NS ROE}
	\bm{J}_{\delta\bm{\alpha}}(t_k) = \frac{\partial \delta\bm{\alpha}}{\partial \delta\bm{\alpha}^\prime} \bigg|_{\delta\bm{\alpha}^\prime = \bm{0}} = 
	\begin{bmatrix} \frac{1}{a_S} & \bm{0}_{1 \times 4} & 0 \\ 0 & \bm{0}_{1 \times 4} & 1 \\ \bm{0}_{4 \times 1} & \textbf{I}_{4 \times 4} & \bm{0}_{4 \times 1} \end{bmatrix},
\end{align}
and $a_S$ is the semi-major axis of the servicer at $t_k$. Noting that $\bm{Q}_{\roe^\prime} = \sum_{i \in \{r, t, n\}} \bm{X}_{k}^{i} {}^\prime \widetilde{Q}_{\roe^\prime}$ as in Eq.~\ref{eqn:Q_roe as sum of diagonal}, the linear mapping matrices of Eq.~\ref{eqn:ASNC Linear Mapping Expanded} are now given as
\begin{align}
	\bm{X}_{k}^i =  \bm{J}_{\delta\bm{\alpha}}(t_k) \bm{X}_{k}^{i} {}^\prime  \bm{J}_{\delta\bm{\alpha}}(t_k)^\top,
\end{align}
where $\bm{X}_{k}^{i} {}^\prime$ of Eq.~\ref{eqn:X matrix def - general} for $\roe^\prime$ is derived by \citet{Stacey2022CovModel} and partially reproduced in Appendix \ref{appendix:Process Noise Models ROE}.

%%%%%%%%%
\subsection{Attitude State Process Noise}

In order to derive the process noise model for the attitude states, STM ($\bm{\Phi}_{\bm{q}, k}$) and the process noise mapping matrix ($\bm{\Gamma}_k$) must first be constructed. First, the dynamics of the MRP vector is given as \cite{Tweddle2015MEKF}
\begin{align}
	\delta\dot{\bm{p}} &= \bigg(-\frac{1}{2}[\bm{w}_{T/S}^T]_\times + \frac{1}{8} (\bm{w}_{T/S}^T)^\top \delta\bm{p}\bigg) \delta\bm{p} + \bigg( 1 - \frac{1}{16}\delta\bm{p}^\top \delta\bm{p}\bigg)\bm{w}_{T/S}^T,
\end{align}
where $[\bm{w}]_\times \in \mathbb{R}^{3 \times 3}$ denotes a skew-symmetric cross product matrix of $\bm{w}$, and the dynamics of relative angular velocity is given in Eq.~\ref{eqn:relative ang vel dynamics}. In MEKF and USQUE frameworks, the MRP vector corresponding to the error-quaternion state is reset to zero prior to each propagation step. Therefore, assuming short propagation intervals and small relative angular velocity, the MRP dynamics equation simplifies to 
\begin{align} \label{eqn:mrp dynamics - approx}
	\delta\dot{\bm{p}} \approx  -\frac{1}{2} [\bm{w}_{T/S}^T]_\times \delta\bm{p} + \bm{w}_{T/S}^T = \frac{1}{2} [\bm{w}_{S/T}^T]_\times \delta\bm{p} - \bm{w}_{S/T}^T,
\end{align} 
where $\bm{w}_{S/T}^T$ = $-\bm{w}_{T/S}^T$, and the second-order terms $(\bm{w}_{T/S}^T)^\top \delta\bm{p}$ and $\delta\bm{p}^\top \delta\bm{p}$ are both assumed negligible. Likewise, the relative angular velocity dynamics in Eq.~\ref{eqn:relative ang vel dynamics} approximates to 
\begin{align} \label{eqn:rel ang vel dynamics - approx}
	\dot{\bm{w}}_{S/T}^T \approx -[\bm{w}_T^T]_\times \bm{w}_{S/T}^T  - \bm{I}_T^{-1} \bm{\varepsilon}_T + \dot{\bm{w}}_S^T,
\end{align}
where the term $\bm{w}_T^T \times \bm{I}_T \bm{w}_T^T$ is assumed negligible, which is a reasonable assumption for a small spin rate and exact if the target spins about one axis. In Eq.~\ref{eqn:rel ang vel dynamics - approx}, $\bm{\varepsilon}_T \in \mathbb{R}^3$ accounts for the unmodeled torque in the system expressed in the target's principal axes frame, and $\dot{\bm{w}}_S^T = R_{T/S} \bm{I}_S^{-1} (\bm{m}_{S} - \bm{w}_{S}^S \times \bm{I}_S \bm{w}_{S}^S)$ is due to Euler's rotational equation. Now, the continuous-time dynamics can be constructed from Eqs.~\ref{eqn:mrp dynamics - approx}, \ref{eqn:rel ang vel dynamics - approx},
\begin{align}
	\begin{bmatrix} \delta\dot{\bm{p}} \\ \dot{\bm{w}}_{S/T}^T \end{bmatrix} = \bm{A} \begin{bmatrix} \delta\bm{p} \\ \bm{w}_{S/T}^T \end{bmatrix}  + \bm{\Gamma} \bm{\varepsilon}_T + \bm{C} = \begin{bmatrix} \frac{1}{2}[\bm{w}_{S/T}^T]_\times & -\bm{I}_{3 \times 3} \\ \bm{0}_{3 \times 3} & -[\bm{w}_T^T]_\times \end{bmatrix} \begin{bmatrix} \delta\bm{p} \\ \bm{w}_{S/T}^T \end{bmatrix} + \begin{bmatrix} \bm{0}_{3 \times 3} \\ -\bm{I}_T^{-1} \end{bmatrix} \bm{\varepsilon}_T + \begin{bmatrix} \bm{0}_{3 \times 1} \\ \dot{\bm{w}}_S^T \end{bmatrix},
\end{align}
where $\bm{A}$ is the plant matrix, and $\bm{\Gamma}$ is the process noise mapping matrix. Then, the following STM can be obtained via zero-hold integration \cite{Tweddle2015MEKF},
\begin{align}
	\bm{\Phi}_{\bm{q}, k}(t,0) = \begin{bmatrix} e^{\frac{1}{2} [\bm{w}_{S/T, k}^T]_\times t} & -\int_{0}^{t} e^{\frac{1}{2} [\bm{w}_{S/T, k}^T]_\times \tau} d\tau \\ \bm{0}_{3 \times 3} & e^{-[\bm{w}_{T,k}^T]_\times t} \end{bmatrix},
\end{align}
which leads to 
\begin{align} \label{eqn:Gamma_bar for attitude, raw with matrix exp}
	\bm{\bar{\Gamma}}_k(t, 0) = \bm{\Phi}_{\bm{q}, k}(t, 0) \bm{\Gamma}_k = \begin{bmatrix} \int_{0}^{t} e^{\frac{1}{2} [\bm{w}_{S/T, k}^T]_\times \tau} d\tau \\ -e^{-[\bm{w}_{T,k}^T]_\times t}  \end{bmatrix} \bm{I}_T^{-1} = \begin{bmatrix} \bm{\Lambda}_1(t) \\ -\bm{\Lambda}_2(t) \end{bmatrix} \bm{I}_T^{-1}.
\end{align}
In order for $\bar{\bm{\Gamma}}_k$ to be used in Eq.~\ref{eqn:X matrix def - general} to compute the linear mapping matrix $\bm{X}_{k}^i$ for $i \in \{x, y, z\}$, the integral of the matrix exponential must be evaluated. From Rodrigues' formula, the exponential of a real, skew-symmetric matrix $\bm{A} = [\bm{a}]_\times \in \mathbb{R}^{3 \times 3}$ is given as
\begin{align}
	e^{\bm{A}} = \textbf{I}_{3 \times 3} + \sin \theta \bm{\hat{A}} + (1 - \cos \theta) \bm{\hat{A}}^2,
\end{align}
where $\theta = \| \bm{a} \|$, and $\bm{\hat{A}} = \bm{A} / \theta$. Applying this to the integrand of the integral term in Eq.~\ref{eqn:Gamma_bar for attitude, raw with matrix exp} yields
\begin{align}
	e^{\frac{1}{2}[\bm{w}_1]_\times \tau} = \textbf{I}_{3 \times 3} + \sin \frac{w_1\tau}{2} [\bm{\hat{w}_1}]_\times + \bigg( 1 - \cos \frac{w_1\tau}{2} \bigg)[\bm{\hat{w}}_1]_\times^2,
\end{align}
where $\bm{w}_1$ is a shorthand notation for $\bm{w}_{S/T, k}^T$, $w_1 = \| \bm{w}_1 \|$, and $[\bm{\hat{w}}_1]_\times = [\bm{w}_1]_\times / w_1$. Integrating over $[0, t]$, one obtains
\begin{align}
	\bm{\Lambda}_1(t) = \int_0^t e^{\frac{1}{2}[\bm{w}_1]_\times \tau} d\tau = \textbf{I}_{3 \times 3}t + \frac{2}{w_1}\bigg( 1 - \cos\frac{w_1t}{2}\bigg) [\hat{\bm{w}}_1]_\times + \bigg(t - \frac{2}{w_1} \sin\frac{w_1 t}{2} \bigg) [\hat{\bm{w}}_1]_\times^2.
\end{align}
Likewise, 
\begin{align}
	\bm{\Lambda}_2(t) = e^{-[\bm{w}_{T,k}^T]_\times t} = \textbf{I}_{3 \times 3} - (\sin w_2 t) [\bm{\hat{w}}_2]_\times + ( 1 - \cos w_2 t) [\bm{\hat{w}}_2]_\times^2,
\end{align}
where $\bm{w}_2$ is a shorthand notation for $\bm{w}_{T,k}^T$. The $\bm{X}_{k}^i$ matrix in Eq.~\ref{eqn:X matrix def - general} can now be computed as
\begin{align} \label{eqn:X matrix for attitude in A, B, C}
	\bm{X}_{k}^i = \bm{I}_{T,i}^{-2} \begin{bmatrix} \bar{\bm{A}}_i  & -\bar{\bm{B}}_i \\ -\bar{\bm{B}}_i^\top & \bar{\bm{C}}_i \end{bmatrix} 
\end{align}
where $\bm{I}_{T,i}$ is the $i$-th diagonal element of $\bm{I}_T$, and the analytical expression for the sub-matrices $\bar{\bm{A}}_i, \bar{\bm{B}}_i, \bar{\bm{C}}_i \in \mathbb{R}^{3 \times 3}$ are provided in Appendix \ref{appendix:Process Noise Models Attitude}.

In summary, the above formulations allow for accurate modeling of the process noise covariance matrix associated with the relative attitude motion based on the underlying continuous dynamics. The assumptions are representative and benign for the purpose of deriving analytical expressions which enable the least-squares minimization problem of ASNC in Eq.~\ref{eqn:ASNC LS minimizaiton}.
